Dialog act guided contextual adapter for personalized speech recognition

Personalization in multi-turn dialogs has been a long standing challenge for end-to-end automatic speech recognition (E2E ASR) models. Recent work on contextual adapters has tackled rare word recognition using user catalogs. This adaptation, however, does not incorporate an important cue, the dialog act, which is available in a multi-turn dialog scenario. In this work, we propose a dialog act guided contextual adapter network. Specifically, it leverages dialog acts to select the most relevant user catalogs and creates queries based on both -- the audio as well as the semantic relationship between the carrier phrase and user catalogs to better guide the contextual biasing. On industrial voice assistant datasets, our model outperforms both the baselines - dialog act encoder-only model, and the contextual adaptation, leading to the most improvement over the no-context model: 58% average relative word error rate reduction (WERR) in the multi-turn dialog scenario, in comparison to the prior-art contextual adapter, which has achieved 39% WERR over the no-context model.

==> EB+DA - ICASSP 2023 camera ready/abstract.tex <==
\begin{abstract}
% Personalization has been a long standing challenge for end-to-end automatic speech recognition (E2E ASR) models in multi-turn dialogs. Recent work on the contextual adapter has tackled personalized rare word recognition with user catalogs, while the dialog act is beneficial for generic ASR in the multi-turn scenario. In this work, we take a further step to explore how they can be complementary with each other and propose a dialog act guided contextual adapter network. Specifically, it leverages dialog acts to select the most relevant catalogs and create queries based on the audio embeddings as well as the semantic relation between carrier phrases and personalized words to better guide the contextual biasing. On industrial voice assistant datasets, our model outperforms the baselines using only the dialog act, and the prior-art contextual adapter, leading to the most improvement, with $58\%$ word error rate relative reduction over the no-context model, in the multi-turn dialog scenario.


Personalization in multi-turn dialogs has been a long standing challenge for end-to-end automatic speech recognition (E2E ASR) models. Recent work on contextual adapters has tackled rare word recognition using user catalogs. This adaptation, however, does not incorporate an important cue, the dialog act, which is available in a multi-turn dialog scenario. %where different user catalogs might be relevant depending on the turn. 
In this work, we propose a dialog act guided contextual adapter network. Specifically, it leverages dialog acts to select the most relevant user catalogs and creates queries based on both -- the audio as well as the semantic relationship between the carrier phrase and user catalogs to better guide the contextual biasing. On industrial voice assistant datasets, our model outperforms both the baselines - dialog act encoder-only model, and the contextual adaptation, leading to the most improvement over the no-context model: 58\% average relative word error rate reduction (WERR) in the multi-turn dialog scenario, in comparison to the prior-art contextual adapter, which has achieved 39\% WERR over the no-context model.



\end{abstract}

==> EB+DA - ICASSP 2023 camera ready/background.tex <==
\section{Contextual Adapter}
\label{sec:bg}

\newcommand{\cnemb}{c^e_i}
\newcommand{\cn}{c_i}
\newcommand{\cni}[1]{c_{#1}}
\newcommand{\cniemb}[1]{c_{#1}^e}
\newcommand{\call}{C}
\newcommand{\cemball}{\boldsymbol{C}^e}
\newcommand{\attni}{\boldsymbol{\alpha}_t}
\newcommand{\attnit}{\alpha_i^t}
\newcommand{\dotprod}{\cdot}
\newcommand{\rootd}{\sqrt{d}}
\newcommand{\querylin}{\boldsymbol{W}^{q}}
\newcommand{\keylin}{\boldsymbol{W}^{k}}
\newcommand{\vallin}{\boldsymbol{W}^v}
\newcommand{\accousticquery}{q}
\newcommand{\semanticquery}{h_u^{pre}}
\newcommand{\encattncont}{b_t^{enc}}
\newcommand{\biasvector}{b}
\newcommand{\encbiasvector}{b^{enc}_t}
\newcommand{\decbiasvector}{b^{pre}_u}
\newcommand{\jointbiasvector}{b_{t,u}}
\newcommand{\jhat}{\hat{j}_{t,u}}
\newcommand{\maxcatsize}{K}
\newcommand{\htcap}{\hat{h}_t^{enc}}
\newcommand{\hucap}{\hat{h}_u^{pre}}
\newcommand{\nobias}{\textit{\textless no\_bias\textgreater} }
\newcommand{\encout}{h_t^{enc}}
\newcommand{\decout}{h_u^{pre}}
\newcommand{\decinp}{y_{u-1}}
\newcommand{\encinp}{x_{t}}
\newcommand{\encinpstart}{x_{0}}
\newcommand{\decinpstart}{y_{0}}
\newcommand{\catlen}{K}
\newcommand{\catembsize}{D}
\newcommand{\fullcatalog}{$\call = [\cni{1}, \cni{2}, \dots, \cni{K}]$}
\newcommand{\fullcatalogemb}{$\cemball = [\cniemb{1}, \cniemb{2} \dots \cniemb{K}]$}
\newcommand{\notype}{\textit{\textless no\_type\textgreater} }

The contextual adapter used in this work,~\cite{sathyendra2022contextual}, is built upon a type of streaming E2E ASR, RNN-T \cite{graves2012sequence}, which consists of an RNN based encoder, an RNN based prediction network, and a joint network. The encoder network produces high-level representations $\mathbf{h}_t^{enc}$ for the audio frames, while the prediction network encodes the previously predicted word-pieces and produces the output $\mathbf{h}_u^{pre}$. The joint network fuses $\mathbf{h}_t^{enc}$ and $\mathbf{h}_u^{pre}$ via the join operation followed by a series of dense layers with activations and a softmax function to obtain the probability distribution over word-pieces plus a $blank$ symbol. In~\cite{sathyendra2022contextual}, a catalog encoder is introduced to embed the user catalogs and types. In addition, a multi-head attention based biasing network is introduced to measure the relevance of the user catalog context using the encoder network outputs as queries. 
%We refer readers to ~\cite{sathyendra2022contextual} for more details.

%The sequence-to-sequence neural transducer is a type of streaming E2E ASR \cite{graves2012sequence}, typically consisting of an encoder network, a prediction network, and a joint network. The encoder network produces high-level representations $\encout$ for the audio frames $\mathbf{x_{0,t}}= (\encinpstart \dots \encinp)$. The prediction network encodes the previously predicted word-pieces $\mathbf{y_{0,u-1}}=(\decinpstart \dots \decinp)$ and produces the output $\decout$. The encoder and prediction network are typically stacked RNN layers \cite{graves2012sequence}, which leads to its name, RNN-T, where
% \begin{align}
%     \encout & = \text{Encoder}(\mathbf{x_{0,t}}); \quad
%     \decout = \text{PredictionNetwork}(\mathbf{y_{0,u-1}}) 
% \end{align}
%The joint network fuses $\encout$ and $\decout$ via the join operation followed by a series of dense layers with activations and produces the lattice scores (denoted by $z_{t,u}$). A Softmax function is then applied to obtain the probability distribution over word-pieces plus a $blank$ symbol. % as:
%\vspace{-15pt}
% \begin{align}
%     P(y_u|t,u) = \text{Softmax}(z_{t,u})    
%     \label{eqn:posterior}
% \end{align}
%The entire model is trained with the RNN-T loss using the forward-backward algorithm that accounts for all possible alignments between the $T$ acoustic frames and $U$ word-pieces in the ground truth \cite{graves2012sequence}. Intuitively, the encoder network is expected to behave as an acoustic model (AM) while the prediction network behaves as a language model (LM) \cite{he2019streaming}.

==> EB+DA - ICASSP 2023 camera ready/conclusion.tex <==
\section{Conclusion}
We proposed a dialog act guided contextual adapter approach to address personalized ASR in multi-turn dialogs. We leverage DAs to short list the most relevant catalogs and create better queries to guide the biasing network. The experimental results on IVA test sets show that the DA guided CA achieves on average $58\%$ WER relative improvements over the no-context model on the \textit{user-specific} multi-turn test set, in comparison to the prior-art contextual adapter model which achieved $39\%$ over the no-context model.
%and the user catalogs in RNN-T via the DA encoder, the catalog encoder, DA fusion networks, and the biasing network. Our experiments on the IVA test sets show that by the Early-Late DA fusion in the CA stage and with the catalog selection based on DA, CADialNet outperforms the approaches where no context is present. The CADialNet also outperforms the models which only integrates DA or user catalogs. 

==> EB+DA - ICASSP 2023 camera ready/experiments.tex <==
\section{Experiments}



\subsection{Datasets and Evaluation Metrics}
\label{sec:dataset}

We use in-house IVA datasets where audio to transcription paired utterances are de-identified and randomly sampled from more than 20 domains such as \textit{Global}, \textit{Communications}, \textit{SmartHome}, \textit{Weather}, and \textit{Music}. We consider the top 49 frequently occurring DAs in the IVA data sets including the \textit{DefaultDialogAct} (usually associated with the first-turn utterances) and the non-default DAs (associated with more follow-up turns)\footnote{There does not exist an equivalent, publicly available contextual dataset containing both user catalogs and dialog acts in multi-turn dialogue scenario.}. 114k hours of data are used to pre-train the DA-Aware RNN-T. For training the catalog encoder and the biasing network, we use approximately 290 hours of data, containing a mix of \textit{user-specific} and \textit{general} training data with the ratio of 1.5:1 as suggested in~\cite{sathyendra2022contextual}. \textit{User-specific} datasets contain utterances with contact names, device names, and/or device locations. \textit{General} utterances are sampled from the original training data distribution. We evaluate the models and report results on multiple test sets including a 20 hour \textit{User-specific} dataset and a 75 hour \textit{General} dataset.
The \textit{User-specific} test set is further split into the default DA and non-default DA set for further comparisons.
%The non-default DA utterances are associated more with personalized utterances.
To evaluate our model on individual turns of a dialog, we further created turn-wise test sets, which contain \textit{user-specific} and non-default DA utterances from the first turn (turn 1), the second turn (turn 2) and the third turn (turn 3). 

The relative word error rate reduction (WERR) is used throughout the experiments to summarize the overall, slot-type-wise, or turn-wise ASR performances. Given a model A's WER ($\text{WER}_A$) and a baseline B's WER ($\text{WER}_B$), the WERR of A over B can be computed by $(\text{WER}_B - \text{WER}_A) / \text{WER}_B$; a higher WERR indicates a better WER. We use three types of catalogs (Section~\ref{sec:da_based_cs}). The maximum number of catalog entities fed into the catalog encoder is set to $K=500$, and contains the correct \textit{user-specific} entities. %\kms{\st{Note that we assume the target personalized words are always present in the catalog both during training and inference}}.

\subsection{Experimental Setup}
\subsubsection{Model Configurations}
The DA guided contextual adapter has the following configuration. The encoder network has 5 LSTM layers and the prediction network is composed of 2 LSTM layers, both with 736 units followed by a feed-forward network of 512 units. The joint network is a fully-connected feed-forward component with one hidden layer followed by a $\tanh$ activation function. The DA encoder contains a 49-dim embedding layer followed by a feed-forward network of 64 units (i.e., $d_{da}=64$). The DA late fusion network has a feed-forward network of 512 units. The catalog encoder is a BiLSTM layer with 128 units (each for forward and backward LSTMs) with input size 64. The final output from the catalog encoder is projected to 64-dim (i.e., $D_{c}=64$). The biasing network projects the query, key and values to 64-dimensions (i.e., $d=64$). The resulting biasing vector is then projected to the same size as the encoder output, 512-dim (i.e., $D_{a}=512$).

We compare our model to the following baselines: (1) \textbf{No Context}: This is a vanilla RNN-T\cite{graves2012sequence}. (2) \textbf{DA only}: This is an RNN-T using only DAs integrated with the input audio features~\cite{wei2021attentive}, and (3) \textbf{CA}: This is an RNN-T based Contextual Adapter (CA) using only user catalogs ~\cite{sathyendra2022contextual}. All the models including the proposed one contain $\sim 35$ million parameters.

% Table 1: WER on P13N and non-P13N - Extended catalog test sets 
\begin{table}[t]
\centering 
\small
\tabcolsep=0.1cm
\caption{WERRs (\%) over No-context baseline~\cite{graves2012sequence}: Comparisons for DA guided CA, DA only, and CA models on IVA \textit{User-specific} and \textit{General} test sets. A higher number indicates a better WER.}
\label{tab:wers_on_p2a}
\resizebox{1.0\linewidth}{!}{%
\begin{tabular}{c|c|c|c|c}
\toprule
Model & DA Fusion & DA Enc.\&FN & User-Specific & General \\ \midrule
% \multirow{3}{*}{DA-aware RNN-T~\cite{wei2021attentive}} & Early Fusion &  & & \textcolor{blue}{\textbf{1.49}} & -0.95 \\
%  & Late Fusion  &  - &  - & -0.07 & -1.16\\
%  & Early-Late Fusion  & & & 0.74 & -1.74 \\ \hline
No context~\cite{graves2012sequence} & N/A & N/A & baseline & baseline \\ \hline
DA Only~\cite{wei2021attentive} & N/A & N/A & 1.49 & -0.95 \\ \hline
CA~\cite{sathyendra2022contextual} & N/A & N/A & 28.23 & -0.59 \\ \hline
% \multirow{2}{*}{CA RNN-T~\cite{sathyendra2022contextual}} & - & \xmark & - & 28.23 & -0.59 \\
%  & -  & \textcolor{blue}{\cmark} &  - & \textcolor{blue}{\textbf{28.90}} & -0.51 \\ \hline
\multirow{6}{*}{\textbf{DA guided CA (Ours)}} & Early Fusion  & freeze & 29.72 & -1.02 \\
 &   & un-freeze & 28.83 & -0.66 \\ \cline{2-5}
 & Late Fusion  & freeze & 28.75 & -1.31 \\
 &   & un-freeze & 30.61 & -2.58 \\ \cline{2-5}
 & Early-Late Fusion & freeze & 30.53 & -2.3 \\
 &   & un-freeze & \textbf{32.39} & -2.5 \\
 \bottomrule
\end{tabular}}%
\vspace{-4.5mm}
\end{table}

\subsubsection{Input, Output, and Learning Rate Configurations}
The input audio features consists of 64-dim LFBE features, which are extracted every 10 ms with a window size of 25 ms from audio samples. The features of each frame are then stacked with the left two frames, followed by a downsampling of factor 3 to achieve low frame rate, resulting in 192 feature dimensions.
The subword tokenizer \cite{sennrich-etal-2016-neural, kudo2018subword} is used to create tokens from the transcriptions; we use 4000 tokens in total. 
We trained the RNN-T, the DA encoder, and the DA fusion network by minimizing the RNN-T loss~\cite{graves2012sequence} using the Adam optimizer \cite{kingma2014adam}, and varied the learning rate following \cite{Dong2018SpeechTransformerAN,NIPS2017_3f5ee243}.with the starting LR = 1.5e-7 and ramping up for $3000$ steps to reach LR = 4e-4. The LR is then held constant for $150K$ steps after which there is an exponential decay. For training the catalog encoder and biasing network in the CA stage, we use the Adam optimizer with LR = 1e-3 trained to convergence with early stopping.

\subsection{Results}

% Table 2: WER on Default DialogAct and Non-Default DialogAct P13N test sets
\begin{table}[t]
\centering
\small
\tabcolsep=0.1cm
\caption{WERRs (\%) over No-context baseline~\cite{graves2012sequence} on Non-Default/Default DA splits of the \textit{User-specific} test set. A higher number indicates a better WER.}
\label{tab:wers_on_da}
\resizebox{1.0\linewidth}{!}{%
\begin{tabular}{c|c|c|c|c}
\toprule
Model & DA Fusion & DA Enc.\&FN & Non-Default DA & Default DA \\ \midrule
No context~\cite{graves2012sequence} & N/A & N/A & baseline & baseline \\ \hline
DA Only~\cite{wei2021attentive} & N/A & N/A & 13.81 & -1.27 \\ \hline
CA~\cite{sathyendra2022contextual} & N/A  & N/A & 29.91 & 27.85 \\ \hline
% \multirow{2}{*}{CA RNN-T~\cite{sathyendra2022contextual}} & - & \xmark & - & 29.91 & 27.85 \\
%  & -  & \textcolor{blue}{\cmark} &  - & \textcolor{blue}{\textbf{30.66}} & \textcolor{blue}{\textbf{28.27}} \\ \hline
\multirow{6}{*}{\textbf{DA guided CA (Ours)}} & Early Fusion  & freeze & 40.35 & 27.77 \\
 &    & un-freeze & 39.71 & 26.84 \\ \cline{2-5}
 & Late Fusion  & freeze & 39.01 & 27.00 \\
 &    & un-freeze & 39.54 & 29.03 \\ \cline{2-5}
 & Early-Late Fusion & freeze & 40.04 & 28.69 \\
 &  & un-freeze & \textbf{41.56} & \textbf{30.46} \\
 \bottomrule
\end{tabular}}%
\vspace{-5.5mm}
\end{table}

\begin{figure}%[h]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/slot_werrs.pdf}
    \vspace{-14pt}
    \caption{Slot WERRs (\%) over No-Context model~\cite{graves2012sequence} on the IVA \textit{User-specific} test set.}
    \label{fig:slot_werrs}
    \vspace{-10pt}
    %\vspace{0.5cm}
\end{figure}

% Table 3: Slot WERs on personalized slots
% \begin{table}[t]
% \centering
% \tabcolsep=0.1cm
% \caption{Slot WERRs (\%) over No-Context model~\cite{graves2012sequence} on the IVA personalized test set}
% \label{tab:wers_on_slots}
% \resizebox{1.0\linewidth}{!}{%
% \begin{tabular}{c|c|c|c|c}
% \toprule
% Slot type & No Context~\cite{graves2012sequence} & DA Only~\cite{wei2021attentive} & CA~\cite{sathyendra2022contextual} & \textbf{DA guided CA (Ours)} \\ \midrule
% Overall (131 slots) & baseline & 1.50 & 28.57 & \textbf{33.08} \\ %\midrule
% Contact Name & baseline & 5.32 & 38.12 & \textbf{45.21} \\ 
% Device Name & baseline & -0.38 & 34.73 & \textbf{38.55} \\ 
% Device Location & baseline & -1.82 & 34.55 & \textbf{36.36} \\
% \bottomrule
% \end{tabular}}%
% \vspace{-2.5mm}
% \end{table}

Table~\ref{tab:wers_on_p2a} presents the WERRs of the DA guided CA and baseline approaches over the no-context model for the \textit{User-specific} and \textit{General} test sets. The DA guided CA 
%(with Early-Late fusion and unfreeze DA Enc. and FN) 
outperforms the no-context model by $32.39\%$ relative improvement, while the DA only model and CA achieve $1.49\%$, and $28.90\%$ WERRs respectively on the \textit{User-specific} set. 
%the proposed model leads to a slight degradation ($\leq2.58\%$) on the \textit{General} set. 
% Interestingly, while early DA fusion leads to the best performing DA-aware RNN-T model, the Early-Late DA fusion is better than late fusion and early fusion in CADialNet. It can be attributed to the continual fine-tuning of the DA fusion network during contextual adaptation, which has the direct impact on the quality of the queries used in the biasing network. 
While unfreezing the DA Enc. and FN boosts the performance on the \textit{User-specific} sets, it is more prone to overbiasing, resulting in more degradations on the \textit{General} set compared to freezing their weights: -1.31\% WERR (freeze) vs. -2.58\% WERR (unfreeze) for the late dialog act fusion, and -2.3\% WERR (freeze) vs. -2.5\% WERR (unfreeze) for the early-late dialog act fusion in Table~\ref{tab:wers_on_p2a}.
We also observe that bypassing the catalog selection with DAs on the best performing DA guided CA, the WERR over No-Context model drops from $32.39\%$ to $31.43\%$, which indicates selecting catalogs and filtering catalog embeddings, i.e. keys/values, to the most relevant ones, leads to better biasing.

In Table~\ref{tab:wers_on_da}, we show the WERRs on non-default DA and default DA splits. The DA guided CA, again, improves WER over the No-Context model the most ($41.56\%$), compared to the WERRs achieved by the DA only ($13.81\%$) and CA ($29.91\%$) on the non-default DA split. The huge improvements seen in the non-default DA split can be explained by the fact that the \textit{user-specific} utterances are usually associated with non-default DA. 
%The larger performance gain compared to Table~\ref{tab:wers_on_p2a} can also be seen for the DA only model over the no-context model ($13.81\%$ vs. $1.49\%$ WERR). 
%Again, the CS, the dialogue-aware encoder outputs, the continual training of DA fusion network are consistently helping the CA RNN-T and CADialNet model for the majority of the settings.

We further compute the slot WERRs on three major \textit{user-specific} slots in Fig.~\ref{fig:slot_werrs}
%Table~\ref{tab:wers_on_slots}
along with the overall performances across all 131 slots. The DA guided CA model shows the most relative improvements in terms of Overall Slot WER against the No-Context model ($33.08\%$), compared to the WERRs of DA Only ($1.5\%$), and CA ($28.57\%$) respectively. Here, we can see the improvements on the contact name slot are the highest across all models. The proposed model achieves the most improvement ($45.21\%$ relative). Notably, although DA Only model performs slightly worse than the No-Context model for the device name and device location slots ($-0.38\%$ and $-1.82\%$ WERRs), DA guided CA still leads to better relative improvement over No-Context model, compared to the CA's improvement for the device name ($38.55\%$ vs. $34.73\%$) and device location slots ($36.36\%$ vs. $34.55\%$) respectively.


\begin{figure}%[h]
    \centering
    \includegraphics[width=0.9\linewidth]{figs/turn_wise_werrs.pdf}
    \vspace{-14pt}
    \caption{Turn-wise WERRs (\%) over No-context baseline~\cite{graves2012sequence} on the IVA \textit{User-specific} multi-turn test set.}
    \label{fig:turn_wise_werrs}
    \vspace{-10pt}
    %\vspace{0.5cm}
\end{figure}
% Table 3: Turn-wise WERs on personalized slots
% \begin{table}[t]
% \centering
% \tabcolsep=0.1cm
% \caption{Turn-wise WERRs (\%) over No-context baseline~\cite{graves2012sequence}: Comparisons on the IVA personalized multi-turn test set}
% \label{tab:wers_on_turns}
% \resizebox{1.0\linewidth}{!}{%
% \begin{tabular}{c|c|c|c|c}
% \toprule
% Turn ID & No-context~\cite{graves2012sequence} & DA Only~\cite{wei2021attentive} & CA~\cite{sathyendra2022contextual} & \textbf{DA guided CA (Ours)} \\ \midrule
% Average & baseline & 18.21 & 39.03 & \textbf{57.96} \\
% Turn 1 & baseline & 19.50 & 37.28 & \textbf{56.53} \\ %\midrule
% Turn 2 & baseline & 18.59 & 41.22 & \textbf{57.35} \\
% Turn 3 & baseline & 16.73 & 38.37 & \textbf{59.77} \\
% \bottomrule
% \end{tabular}}%
% \vspace{-2.5mm}
% \end{table}


\begin{comment}
% Table 3: Slot WERs on personalized slots
\begin{table}[h]
\centering
\tabcolsep=0.1cm
\caption{Slot WERRs (\%) over Vanilla RNN-T on the IVA personalized test set.}
\label{tab:wers_on_slots}
\resizebox{1.0\linewidth}{!}{%
\begin{tabular}{c|c|c|c|c}
\toprule
Slot type & Vanilla RNN-T~\cite{graves2012sequence} & DA-aware RNN-T~\cite{wei2021attentive} & CA RNN-T~\cite{sathyendra2022contextual} & \textbf{CADialNet (Ours)} \\ \midrule
Overall (131 slots) & 0 & 1.50 & 28.57 & \textbf{33.08} \\ %\midrule
Contact Name & 0 & 5.32 & 38.12 & \textbf{45.21} \\ 
Device Name & 0 & -0.38 & 34.73 & \textbf{38.55} \\ 
Device Location & 0 & -1.82 & 34.55 & \textbf{36.36} \\
\bottomrule
\end{tabular}}%
\vspace{-2.5mm}
\end{table}
\end{comment}

\begin{comment}
% Table 3: Turn-wise WERs on personalized slots
\begin{table}[h]
\centering
\tabcolsep=0.1cm
\caption{Turn-wise WERRs (\%) over Vanilla RNN-T on the IVA personalized, non-default DA test set.}
\label{tab:wers_on_turns}
\resizebox{1.0\linewidth}{!}{%
\begin{tabular}{c|c|c|c|c}
\toprule
Turn ID & Vanilla RNN-T~\cite{graves2012sequence} & DA-aware RNN-T~\cite{wei2021attentive} & CA RNN-T~\cite{sathyendra2022contextual} & \textbf{CADialNet (Ours)} \\ \midrule
Turn 1 & 0 & 19.50 & 37.28 & 56.53 \\ %\midrule
Turn 2 & 0 & 18.59 & 41.22 & 57.35 \\
Turn 3 & 0 & 16.73 & 38.37 & 59.77 \\
\bottomrule
\end{tabular}}%
\vspace{-2.5mm}
\end{table}
\end{comment}

Finally, we report the results on the turn-wise
%, personalized, non-default dialogue act 
test sets in Fig.~\ref{fig:turn_wise_werrs}.
%Table~\ref{tab:wers_on_turns}. 
The average of WERRs across turns are presented as well. While the DA Only model and CA have significant improvements, 
%on average, $18.2\%$ and $39.0\%$ WERR, respectively, 
DA guided CA leads to the best improvements on average ($58\%$), turn 1 ($56.5\%$), turn 2 ($57.3\%$), and turn 3 ($59.8\%$) over the No-Context model. This shows that the DA guided CA model significantly improves performances for multi-turn personalized ASR over the baselines.

==> EB+DA - ICASSP 2023 camera ready/introduction.tex <==
\section{Introduction}
\label{sec:intro}

Personalized speech recognition has gained considerable attention in recent years as industrial voice assistants (IVAs) rise in popularity.
To provide the best customer experience, 
an IVA should be able to recognize personalized requests correctly. For example, \textit{``drop in on [Proper Name]''}, where the name could be user defined words. 
 
End-to-end deep neural networks have become the mainstream approach for ASR in IVAs, due to their great capacity to learn the audio-to-text mapping without the alignment information between the audio and text transcript~\cite{chiu2018state}. These systems include the Connectionist Temporal Classification (CTC) \cite{Graves2006ConnectionistTC}, Listen-Attend-Spell (LAS)\cite{LAS2016}, Recurrent Neural Network Transducer (RNN-T) \cite{graves2012sequence}, and the transformer network \cite{Dong2018SpeechTransformerAN}. 
However, E2E ASR models face challenges in generalizing to recognize user-specific rare words,
% tokens in the distribution tail, 
such as contact names, proper nouns, and named entities due to the scarcity of paired audio-to-text training data~\cite{bruguier2016learning,sainath2018no,pundak2018deep,chen2019joint,bruguier2019phoebe}.
 
Prior works have explored various types of contextual information to improve personalized speech recognition~\cite{Mohri2002WeightedFT,williams2018contextual,liu2021domainaware,jain2020contextual,liu2020contextualizing,chang2021context,sathyendra2022contextual,pundak2018deep, gourav2021personalization}: The weighted finite state transducers (WFSTs)~\cite{Mohri2002WeightedFT} on the rare words \cite{williams2018contextual}; Domain-aware neural language models~\cite{liu2021domainaware}; Text metadata of video~\cite{jain2020contextual,liu2020contextualizing}, and the catalogs~\cite{chang2021context,sathyendra2022contextual} provided by speakers such as contact names and device names. %~\cite{chang2021context,sathyendra2022contextual}
%showed that training-time integration of personalized contexts outperforms the post-training integration.
The contexts are incorporated to the model either with the shallow fusion~\cite{gourav2021personalization,Zhao2019} or the neural biasing approaches \cite{bruguier2019phoebe,pundak2018deep,abro2019multi,chang2021context,sathyendra2022contextual}. The neural solutions have been shown outperforming the use of grammars or dynamic WFSTs in the shallow fusion.
In~\cite{chang2021context,sathyendra2022contextual}, the catalog entities are encoded by BiLSTM or BERT based encoders, and then integrated with the audio encoder via a multi-head attention based contextual biasing network. The model is taught to leverage user-specific contexts to improve the recognition of rare words. The performance of this biasing approach, however, may be hindered when irrelevant user catalogs or/and wrongly predicted carrier phrases bias the next predictions towards a wrong token.
 %For example, the model should not use the device name catalog for an utterance like \textit{``call [Contact Name]''} but only focus on biasing toward the contact name catalog instead.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{figs/high_level_diagram_v3.pdf}
    %\vspace{0pt}
    \vspace{-2.5mm}
    \caption{
    A high-level diagram illustrating our idea to leverage both dialog act and user catalogs to help a voice assistant (VA) recognizing proper nouns in a multi-turn dialog. Note that prior contextual adapters~\cite{chang2021context,sathyendra2022contextual} consider only user catalogs for contextual biasing.
    %Prior contextual adapters~\cite{chang2021context,sathyendra2022contextual} bias utterances without considering the dialog act, which however can be useful to link the intention in the audio with relevant user catalogs as well as next-turn utterances. We work towards addressing this gap in this work.
    }
    \label{fig:da_eb_high_level}
    %\vspace{-6pt}
    \vspace{-0.5cm}
\end{figure}

To address the above issues, we propose to leverage both dialog act and user catalogs for the contextual biasing (Fig.~\ref{fig:da_eb_high_level}) and introduce a dialog act guided contextual adapter network (Fig.~\ref{fig:ca_da}). The dialog acts (DA) are used to identify the action and the slot value of spoken utterances in multi-turn dialogues (Fig.~\ref{fig:da_eb_high_level}). An example of DA is \textit{SlotValueElicitation(ProperName)}, which is associated with a dialog when a user tries to call someone. The DA can help the VA to elicit a contact name from the user catalog for the next turn, usually to clarify or confirm the entity. Given the semantic relationship between ``\textit{drop in on}'' or ``\textit{call}'' versus ``\textit{SlotValueElicitation}", DAs can help improve the prediction of the carrier phrases. We then use an attention based contextual adapter to 
bias the predictions towards the tokens in the user's \textit{[Contact Name]} catalog.
Note that prior work with DAs~\cite{wei2021attentive,kim2019gated,wu2020multistate,gupta2018efficient} primarily focus on the generic multi-turn utterance improvements, while the contextual biasing approaches~\cite{chang2021context,sathyendra2022contextual} were mainly dedicated to the single-turn named entity improvement. With the proposed network, we can bridge the gap between a single turn and multi-turn personalization in ASR. 

%Dialog acts (DAs) have been shown effective to improve the end-to-end ASR model accuracy \cite{wei2021attentive,kim2019gated,wu2020multistate,gupta2018efficient}. An example of DA is \textit{SlotValueElicitation(ProperName)} associated with a dialog when a user tries to call someone. The DA help guiding the VA to elicit a contact name from the user catalog in the next turn, usually to clarify or confirm the entity. Given the semantic relationship between the carrier phrase and DA, e.g. \textit{call} versus \textit{SlotValueElicitation}, DAs can help improve the prediction of the carrier phrases. Using DA only, however, does not bias the predictions towards the tokens in the user catalog entities, as it is done in the contextual adaptation. 
%Given the semantic relationship between the carrier phrase and the dialog act string, just the DA's could help for dialog act specific biasing and improve the prediction of the carrier phrases. However, this does not bias the predictions towards the tokens in the user's \textit{[Contact Name]} catalog, as it is done in the case of contextual adaptation.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.7\linewidth]{figs/eb_da_diagram_v3.pdf}
    %\vspace{0pt}
    \vspace{-2.5mm}
    \caption{\textbf{The proposed DA guided contextual adapter.} The DAs are used for catalog selection and are fused with different levels of audio representations to build better queries for the biasing network.
    %We inject and leverage DA contexts in three ways: (1) Early fusion of DA embeddings with the input audio features (2) Late fusion of DA embeddings with the encoder network outputs, and (3) Catalog selection based on the DA string. The DA fusion network outputs are served as queries (Q) used in the biasing network. Note that the DA early fusion and late fusion can be performed either exclusively or jointly as described in Section~\ref{sec:da_fusion_net}.
    }
    \label{fig:ca_da}
    %\vspace{-6pt}
    \vspace{-0.5cm}
\end{figure*}
 
 %To address the above issues, we propose to leverage the dialog acts, which are tags that help IVA conversations identify the purpose or function of user utterances. For example, the dialog act for the utterance \textit{``call [Contact Name]''} could be annotated as \textit{SlotValueElicitation(ContactName)}.
 %To select the most relevant catalogs for the contextual biasing, we propose to leverage the dialog act, which are prompts that help IVA conversations identify the purpose of user utterances and IVA responses. For example, the dialog act for the utterance \textit{``call [Contact Name]''} is annotated as \textit{SlotValueElicitation(ContactName)}, while \textit{``turn on [Device Name]''} is annotated as \textit{SlotValueElicitation(Appliance)}. Since the dialog act provides the semantic relationship between the carrier phrase and the personalized term, it can not only help select catalogs for the biasing, but also improve the prediction of the carrier phrases.
 %but does not influence directly the prediction of the personalized entity itself. For example, it may prevent \textit{``call [Contact Name]''} being incorrectly predicted as \textit{``call [Device Name]''} but does not affect the prediction for the value of \textit{[Contact Name]} itself.
 
%In this work, we capture the best of these two worlds and introduce a dialog act guided contextual adapter.
%In this work, we introduce an integrated network --  dialog act guided contextual adapter (Fig.~\ref{fig:ca_da}) to bridge the gap between a single turn and multi-turn personalization in ASR. 
Our contributions are summarized as follows. First, we present the dialog act (DA) encoder (Section \ref{sec:da_enc}) and the fusion networks (Section \ref{sec:da_fusion_net}) to integrate the dialog act context with both the low level and high level acoustic representations, and improve the queries for the biasing network. Second, we use dialog acts to select the most relevant catalogs (Section \ref{sec:da_based_cs}), which directly influence the keys/values used in the biasing network. Third, we introduce a DA-aware biasing network, which takes the improved queries and keys/values above to bias toward the right catalog entities (Section \ref{sec:biasing_net}). Finally, we propose a two-stage adapter training and investigate the impacts of freezing and unfreezing DA encoder and fusion networks during the contextual biasing stage (Section \ref{sec:adapter_training}).



 


==> EB+DA - ICASSP 2023 camera ready/proposed_framework.tex <==
\section{Dialog Act Guided Contextual Adapter}
\label{sec:proposed}

In order to leverage DAs to guide the contextual adapter learning, we introduce four new components as shown in Fig.~\ref{fig:ca_da}: (1) DA Encoder, (2) DA Fusion Networks, (3) Catalog selection with DAs, and (4) DA aware Biasing Network, along with the two stage adapter training.

\subsection{DA Encoder}
\label{sec:da_enc}
Each DA string, $\text{d}_i$, contains the action string $\text{a}_i$ and the slot string $\text{s}_i$, in the form of $\text{a}_i(\text{s}_i)$, e.g. \textit{SlotValueElicitation(ProperName)}, as shown in Figure~\ref{fig:da_enc_fusion}(a). Motivated by \cite{wei2021attentive}, we convert $\text{a}_i$ and $\text{s}_i$ by two embedding matrices into the action embeddings $\mathbf{h}_i^{a}$ and slot embeddings $\mathbf{h}_i^{s}$, with the same embedding size. Both embeddings are then fused via an element-wise addition followed by a Feed Forward Network (FFN) and the \text{ReLU} activation, denoted as $\sigma$, to produce the fixed dimensional DA embedding, $\mathbf{h}_i^{DAE} \in \mathbb{R}^{1 \times d_{da}}$: %$\mathbf{h}_i^{DAE} \in \mathbb{R}^{ d_{da} \times 1}$: $\mathbf{h}_i^{DAE} = \sigma(\text{FFN}(\mathbf{h}_i^{a}+\mathbf{h}_i^{s}))$.

\begin{align}
    \vspace{-2.5mm}
    \mathbf{h}_i^{DAE} = \sigma(\text{FFN}(\mathbf{h}_i^{a}+\mathbf{h}_i^{s}))
    \label{eq:da_enc}
    %\vspace{-20.5mm}
\end{align}

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/DA_encoder_and_fusion_network.pdf}
    \vspace{-20pt}
    \caption{\textbf{The DA encoder and fusion networks}. (a) DA encoder, (b) DA early fusion network, and (c) DA late fusion network}
    \label{fig:da_enc_fusion}
    %\vspace{-6pt}
    %\vspace{0.5cm}
    \vspace{-10.5mm}
\end{figure}


% \subsection{Catalog Encoder}
% \label{sec:catalog_enc}
% Given a catalog of contextual entities, 
% \fullcatalog, the catalog encoder produces one encoded representation or \textit{entity embedding, $c_i^e$,} per entity in the catalog. 
% With $\catlen$ entities in the user's catalog and embedding size $\catembsize$, the catalog encoder outputs $C^e \in \mathbb{R}^{K\times D} $. 
% Each entity $c_i$ is first split into fixed-length word-pieces using a sub-word tokenizer \cite{sennrich-etal-2016-neural, kudo2018subword}, then passed through an embedding lookup followed by BiLSTM layers to obtain an entity's \textit{text embedding}, $c_i^{te}$. 
% %The final states of the BiLSTMs are forwarded as the \textit{text embeddings} of the named entities, denoted as $c_i^{te}$ ~where
% % \begin{align}
% %     c_i^{te} = \text{BiLSTM}(\text{Embedding}(c_i))
% %     \label{eq:catalog_enc}
% % \end{align}
% We use the same tokenizer as used by the RNN-T's prediction network to maintain compatibility with the RNN-T's output vocabulary. 

% In order for the contextual adapters to distinguish between different catalog types and bias toward a specific one, we also encode the type of catalog such as contact names, device names, device locations via a learnable \textit{type embedding} (as in \cite{sathyendra2022contextual}). Given the entity $c_i$ and type $t_i \in \tau$ where $\tau$ is the set of entity types, the final \textit{entity embedding} is computed as $\cnemb = \text{Concat}(c_i^{te}, \text{TypeEmbedding}(t_i)))$
% % \begin{align*}
% % \cnemb = \text{Concat}(c_i^{te}, \text{TypeEmbedding}(t_i))).
% % \end{align*}

% Since the catalog entities may not always be relevant (for example, utterances in the \textit{Weather} domain may not need biasing towards device names), we also introduce a special \nobias token associated with a special \notype type into our catalog (as in \cite{pundak2018deep}, \cite{sathyendra2022contextual}). 

\subsection{Fusion of DAs and Multi-level Audio Embeddings}
\label{sec:da_fusion_net}

After we obtain the DA embedding, $\mathbf{h}_i^{DAE}$, it is combined with two levels of the audio representations using one of the three approaches presented below:

\textbf{Early Fusion}: We simply concatenate $\mathbf{h}_i^{DAE}$ with the input audio features per frame, $\mathbf{x}_t$, see Figure~\ref{fig:da_enc_fusion}(b).
%\vspace{-2.5mm}
\begin{align}
    \mathbf{h}_t^{EF} = \text{Concat}(\mathbf{x}_t, \mathbf{h}_i^{DAE})
    \label{eq:early_fusion}
\end{align}

\textbf{Late Fusion}: The encoder network output, $\mathbf{h}_t^{enc}$ is first concatenated with $\mathbf{h}_i^{DAE}$. The concatenated output is then transformed by a FFN with the \text{ReLU} activation, denoted as $\sigma$. See Figure~\ref{fig:da_enc_fusion}(c).
%\vspace{-2.5mm}
\begin{align}
    \mathbf{h}_t^{LF} = \sigma(\text{FFN}(\text{Concat}(\mathbf{h}_t^{enc}, \mathbf{h}_i^{DAE})))
    \label{eq:late_fusion}
\end{align}

\textbf{Early-Late Fusion}: In this approach, we inject $\mathbf{h}_i^{DAE}$ jointly with the input audio (Equation~\ref{eq:early_fusion}) and with the encoder output (Equation~\ref{eq:late_fusion}) as shown in Figure~\ref{fig:ca_da}. Note that the DA encoder is shared in this approach.

\subsection{Catalog Selection with DAs}
\label{sec:da_based_cs}

In addition to fusing the DA embeddings with the audio representations (Section~\ref{sec:da_fusion_net}), we also investigate the selection of catalogs based on the DA string $\text{d}_i=\text{a}_i(\text{s}_i)$, during training. Specifically, the slot string $\text{s}_i$ in $\text{d}_i$ is used for selecting the catalog for biasing. We consider three types of catalogs in this work: contact names, device names, and device locations. By matching $\text{s}_i$ with the catalog type, we can summarize the selection rule as follows:
\vspace{-0.5mm}
\begin{align}
    \small
     \{c_1,...c_K\} \in \begin{cases}
			\text{proper names catalog}, & \text{if $\text{s}_i$ = \textit{ProperName}}\\
			\text{device names catalog}, & \text{if $\text{s}_i$ = \textit{DeviceName}}\\
			\text{device locations catalog}, & \text{if $\text{s}_i$ = \textit{DeviceLocation}}\\
            \text{all three catalogs}, & \text{otherwise}
		 \end{cases} \nonumber
\end{align}

Using this approach, we can prevent irrelevant catalogs from deteriorating biasing network training.


\subsection{DA Aware Biasing Network}
\label{sec:biasing_net}
The biasing network learns which catalog entities to bias toward. Inspired by~\cite{chang2021context,sathyendra2022contextual}, we employ cross-attention to attend over the catalog embedding matrix $\cemball \in \mathbb{R}^{K \times D_c}$ based on the input query $\mathbf{q}$, which comes from the DA late fusion network, $\mathbf{h}_t^{LF} \in \mathbb{R}^{1 \times D_a}$ (Equation~\ref{eq:late_fusion}). Here $K$, $D_c$, $D_a$ are the total number of catalog entities, the catalog embedding size, and the audio embedding size respectively. This query intuitively encodes both the audio and the DA information -- the semantic relationship between the carrier phrase and the user catalogs.

The query and the catalog entity embeddings are first projected via $\querylin \in \mathbb{R}^{D_a \times d}$ and $\keylin \in \mathbb{R}^{D_c \times d}$ to dimension $d$. An attention score vector $\attni$ for catalog entity embeddings is computed by the scaled dot product attention mechanism~\cite{NIPS2017_3f5ee243} as follows: 
\begin{align}
    \attni = \text{Softmax} \left(\frac{(\cemball \keylin) (\mathbf{h}_t^{LF}\querylin)^T}{\rootd} \right)
\end{align}
where $\attni \in \mathbb{R}^{K \times 1}$. The biasing vector $\mathbf{b}_t^{enc}$ is then computed as $\mathbf{b}_t^{enc} = (\attni)^T (\cemball \vallin) \in \mathbb{R}^{1 \times D_a}$, where ${\boldsymbol{W}^{v}} \in \mathbb{R}^{D_c \times D_a}$. The biasing vector $\mathbf{b}_t^{enc}$ is then combined with the $\mathbf{h}_t^{LF}$: $\hat{\mathbf{h}}_t^{enc} = \mathbf{h}_t^{LF} \oplus \mathbf{b}_t^{enc}$.
% \begin{align}
%     \mathbf{b}_t^{enc} & = \text{BiasingNetwork}(\mathbf{h}_t^{LF}, C^e); \quad \hat{\mathbf{h}}_t^{enc} = \mathbf{h}_t^{LF} \oplus \mathbf{b}_t^{enc}
%     %\label{eq:biasing}
%     \nonumber
% \end{align}

While the audio representation enables the biasing network to bias towards entities based on acoustic similarity, the DA helps the biasing network attend over the right \textit{type} of entity. For instance, if the DA is \textit{SlotValueElicitation(DeviceName)}, the biasing network can be guided to bias towards entities that are of type \textit{DeviceName}.


\subsection{Two-Stage Training: DA-Aware RNN-T Training followed by Contextual Adaptation}
\label{sec:adapter_training}

While improving user-specific word recognition, a desirable E2E ASR should be able to maintain the performance on general speech recognition. To this end, we adopt the two-stage training similar to \cite{sathyendra2022contextual}. We first pre-train the DA-Aware RNN-T, i.e. RNN-T (the encoder network, prediction network, joint network, dense layer) augmented with the DA encoder and DA fusion networks on the live IVA distribution of utterances. In the second stage of contextual adaptation on user catalogs, we keep the RNN-T weights frozen while training the catalog encoder and the biasing network on upsampled personalized data mixed with the original general data under two conditions: (1) Freeze the DA encoder (DA Enc.) and fusion network (FN), (2) Unfreeze/ keep finetuning the DA Enc. and FN.
